Computable Caratheodory Theory

Conformal Riemann mapping of the unit disk onto a simply-connected domain $W$ is a central object of study in classical Complex Analysis. The first complete proof of the Riemann Mapping Theorem given by P. Koebe in 1912 is constructive, and theoretical aspects of computing the Riemann map have been extensively studied since. Carath{\'e}odory Theory describes the boundary extension of the Riemann map. In this paper we develop its constructive version with explicit complexity bounds.

==> intro.tex <==

%\section{Skeleton of the story}
%
%\begin{enumerate}
%\item Caratheodory space can be endowed with a computable structure: use ``finite'' sequences of crosscuts or loops to describe rational points and compute caratheodory distance between them by using chains.  
%\item General statement:  $\varphi$ is computable from caratheodory space (as a computable metric space) to the disc.  By recursive compactness, so is $f$. 
%\item In the locally connected case, one can ask whether $f$ is computable w.r.t euclidean metric.  The answer is that $f$ is computable if and only if  both the boundary and  the modulus of connectivity is provided (by an oracle, or it is just computable).  The counterexample being a modulus growing faster than any computable function.
%\item question:  if $f$ is computable, can we compute the modulus? 
%\item It follows that in the loc. connected case, convergence of the Riemann maps has speed of convergence computable from the modulus and the boundary. 
%\item time complexity is also bounded from below by the modulus of continuity, and therefore  arbitrarily high. 
%\end{enumerate}


\section{Introduction}
%
%Let $U$ be a simply connected subset of $\riem$ with infinite complement $\riem - U$. The Riemann Mapping Theorem asserts that there is a conformal isomorphism 
%$$
%\varphi : U\to D,
%$$
%where $D$ is the unit disk. In some cases, $\varphi$ will extend to a homeomorphism from the closure $\bar{U}$ onto the closed disk. 
%
%\begin{theorem}[Caratheodory]The Riemann map $\varphi:U\to D$ extends uniquely to a homeomorphism between the completion $\hat{U}$ and the completion $\hat{D}\sim \bar{D}$.
%\end{theorem}

\subsection{What is this about and why should one care about this stuff} 


\section{The results}
\subsection{Non locally connected case: Caratheodory metric}

The Caratheodory completion $\hat{U}$ can be made a compact metric space with Caratheodory metric, from now on denoted by $d_{C}$.  In order to be handled by a computer, we will represent points in this space by infinite sequences of polygonal crosscuts or loops (each curve being finitely described).   

More precisely, each point $x$ in $\hat{U}$ will be represented by a sequence $\{\gamma_{n}\}$  of curves finitely described.  For points in the interior, the curves will be loops satisfying diam$(\gamma_{n})\leq 2^{-n}$, for every $n$. For points in the boundary, the curves will be crosscuts with the same small diameter property. 

%Thus, given a description $\{\gamma_{n}\}$ of a point $z\in\hat{U}$, we can for instance semi-decide whether $z$ is in the boundary of $\hat{U}$ (a prime end), just by semi-deciding whether $\gamma_{n}(0)\neq \gamma_{n}(1)$.   

With this convention, a point $z\in \hat{U}$ is computable if there is some computable sequence $\{\gamma_{n}\}$ representing it.  Clearly, rational points in ${U}$ are computable points in $\hat{U}$.


At this point we can state our first result. 

\begin{theorem}Assume $U$ is a simply connected domain, and that the Riemann map $\varphi : U\to D$ is computable. Then, from a description $\{\gamma_{n}\}_{n\in \NN}$ of a prime end $P \in \hat{U}$, we can compute an euclidean description of $\varphi(P)\in \bar{D}$.  In particular, the extended map $\hat{\varphi}:\hat{U}\to \bar{D}$ is computable as a map between represented spaces, with the Caratheodory representation for $\hat{U}$.  
\end{theorem}

\begin{proof}By Proposition \ref{Lavrentiev}.
\end{proof}

It is natural to ask whether the Caratheodory metric space can be made computable, so as to have a statement of computability of the extended map between computable metric spaces.  To achieve this, we will further assume that there is a computable sequence $L=s_{n}$ of computable points in $U$ which is dense in $\hat{U}$ (called the ideal points).  In order to make the triple $(\hat{U},L,d_{C})$ a computable metric space, we need to be able to compute the Caratheodory distance $d_{C}(s_{i},s_{j})$ between ideal points, uniformly in $i$ and $j$. 

It is natural to ask what euclidean information is sufficient to compute the  Caratheodory distance between the ideal points of $\hat{U}$. The answer is given by the following result:


\begin{proposition}
Let $U$ be a simply connected domain. Suppose that we are given  $U$ as an open set, and $\partial U$ as a computable closed set (in the Hausdorff sense). Then the triple $(\hat{U},L,d_{C})$ is a computable metric space which is moreover computably compact.  
\end{proposition}

\begin{proof}
Let $s$ and $s'$ be ideal points.  By taking sufficiently smalls loops around $s$ and $s'$, and sufficiently good internal polygonal approximations of $U$, we will eventually find a polygon $P_{n}$ containing $s$ and $s'$. To compute the distance at precision $\varepsilon$, take an even bigger $n$ if necessary so as to have $2^{-n}<(\varepsilon/2M)^{2}$\footnote{I'm not sure if this is enough.}, and compute the diameter of the smallest path joining $s$ to $s'$ in $P_{n}$ at precision $\varepsilon/2$. This is the desired approximation. For the compactness part, the same $\varepsilon$-net that works for $\bar{U}$, works for $\hat{U}$\footnote{right?}. 
\end{proof}

\begin{remark}
To compute the Riemann map $\varphi :U \to D$, we need a description of $U$ as an open set, and a description of its boundary $\partial U$ as a closed set. This information is weaker than the one required by the above proposition.  
\end{remark}


Now we can state the following sharper result. 


\begin{theorem}Under the conditions of the above proposition, both the extension $\hat{\varphi}: \hat{U} \to \bar{D}$ and its inverse $\hat{f}:\bar{D}\to \hat{U}$ are computable, as functions between computable  metric spaces. 
\end{theorem}


\subsection{Locally connected case: Euclidean metric}

In the locally connected case, prime ends correspond to euclidean points. This means that $\hat{f}$ is well defined as a function from $\bar{D}$ to $\bar{U}$, with the euclidean metric on both sides. 

What additional information is required by an algorithm to compute $\hat{f}$ w.r.t. the euclidean descriptions? 


%*********************  TRY NUMBER ONE **********************
%
%\begin{theorem}
%If we have an oracle for the modulus of connectivity, and another oracle for the boundary (in the housdorff sense), then $f:\bar{D}\to \bar{U}$ is computable w.r.t. the euclidean descriptions. 
%\end{theorem}
%
%The proof will follow from the following proposition and Theorem \ref{non locally connected}. 
%
%\begin{proposition}Suppose we have oracles for the following:
%\begin{itemize}
%\item a description of the domain $U$ as a lower-computable open set,
%\item a description of the boundary $\partial U$ as a computable closed set and
%\item a description of the modulus of connectivity $m(\varepsilon)$ as a computable function, 
%\end{itemize}
%then we can compute a description of\,  $\hat{U}$ as computable metric space with Caratheodory metric and a witness for compactness. Moreover, from the Caratheodory description of a point $z\in \hat{U}$, we can recover its euclidean description. 
%\end{proposition}
%
%
%\begin{remark}It remains the question of whether the modulus of continuity can be computed from $f$.  It looks like the answer is negative. Have to built the counterexample. 
%\end{remark}
%
%****************** TRY NUMBER 2 *****************
%
%\begin{itemize}
%\item From a description of the domain by inner polygons, one can compute a complete system of crosscuts (in which crosscuts are finitely described)
%\item If moreover we know $m(\varepsilon)$, then we can compute $\varphi$. 
%\end{itemize}
%
%\begin{proposition}
%Let $U$ be a simply connected domain. Suppose that we are given a sequence of polygons $U_{n}$ with the following property. 
%\begin{itemize}
%\item $U_{n}\subset int(U_{n+1})\subset U$,
%\item for all $x\in \partial U_{n}$ there is $y\in \partial U$ such that $d(x,y)\leq 2^{-n}.$
%\end{itemize}
%Then we can compute, for every $\varepsilon$, a finite collection of crosscuts $\{\gamma_{1},...,\gamma_{m}\}$ covering $\partial U$ such that diam$(\gamma_{i})\leq \varepsilon$. 
%\end{proposition}
%
%\begin{proof}
%Let $\varepsilon >0$. Take $n$ such that $2^{-n}<\varepsilon/10$. Take an $\varepsilon/3$-net of $\partial U_{n}$. For each point $x$ in this net, draw a $\varepsilon/2$-circular crosscut for $\partial U_{n}$.  To extend each of these crosscuts to a crosscut for $\partial U$, just join each endpoint to $\partial U$ by a $\varepsilon/5$ circular arc. 
%\end{proof}
%
%\begin{remark}
%Each crosscut computed above is described by $(a,b,R,r)$ where $a$ and $b$ are ``rational'' points in $\partial U_{n}$, $R$ is the ``radius'' of the  arc joining $a$ and $b$, and $r$ is the radius of the small arcs joining each of the points $a$ and $b$, to $\partial U$. Notice that even if this finite information completely determines the crosscut, it does not give us enough information to actually compute the endpoints. 
%\end{remark}
%
%*********************** TRY NUMBER 3 ***********************************
%

We will show that the required additional information is  captured \emph{exactly} by what we call here the \emph{Caratheodory modulus of the domain}. 

\begin{definition}[Caratheodory modulus]Let $U$ be a simply connected domain. If  $N(\gamma)$ denotes the neighborhood corresponding to a crosscut $\gamma$, then the \emph{Caratheodory modulus} of the domain $U$ at scale $\delta$ is defined by:
$$
\eta(\delta):=\sup \rm diam(N(\gamma))
$$
where the supremum is taken over all the crosscuts $\gamma$ whose diameter is less than $\delta$.
\end{definition}

We remark that $\eta(\delta)\to 0$ as $\delta \to 0$ if and only if $U$ is locally connected\footnote{Reference needed}.  This means that, if we denote by $m(\delta)$ the modulus of local connectivity, then both modulus tend simultaneously to zero. That is, these quantities describe the same geometric property.  Surprisingly, we will see that they are computationally different by showing that the corresponding rates of decay  are computationally incommensurable. 

But first, we show that the Caratheodory modulus is the right object when concerned with computability of the extension to the boundary in the locally connected case. More precisely, we show that the extension  to the boundary $\bar{f}$ of the Riemman map $f$ from the unit disk to a locally connected (and computable) domain $U$, is computable if and only if the Charatheodory modulus has a computable rate decay.   


\begin{theorem}
Suppose that $U$ is a locally connected domain which contains the origin and that $f:D \to U$ maps the unit disk conformally onto $U$ such that $f(0) = 0$. Assume further that $f$ is a computable map. Then the extension to the boundary $\bar{f}:\bar{D}\to \bar{U}$ is computable if and only if the Caratheodory modulus $\eta(\delta)$ has a computable rate decay.  Moreover, there is an algorithm that from a description of $f$ and $\eta$ computes a description of $\bar{f}$. There is also an algorithm performing the opposite task.  
\end{theorem}

\begin{proof}

For $0<r<1$ and $|z_{0}|=1$ define 
$$
w(r,z_{0}):=\sup |f(z_{1})-f(z_{2})|
$$
where the supremum is taken over all $z_{1}$, $z_{2}$ such that $|z_{i}|<1$ and $|z_{i}-z_{0}|<r$.  Then let 
$$
w(r):=\sup_{|z_{0}|=1}w(r,z_{0}).
$$

by Theorem 1 of Warshawsky, we know that 
$$
w(r)\leq \eta\left( \left(\frac{2\pi A}{\log 1/r}  \right)^{1/2}\right)
$$
where $A$ is an upper bound on the area of the domain $U$.  Assume we have descriptions of $f$ and $\eta$\footnote{Of course, we only need a decreasing upper bound}.

 Let $z\in \bar{U}$ and $\varepsilon>0$.  We now show how to compute $\bar{f}(z)$ at precision $\varepsilon$.  Start by choosing a computable but not rational number $r$ such that 
 $$
 \eta\left( \left(\frac{2\pi A}{\log 1/(2r)}  \right)^{1/2}\right) < \frac{\varepsilon}{2}.
 $$

Then take a rational  approximation $z'$ of $z$ such that $|z-z'|<r/10$.  Since $|z'|\neq 1-r$, we can decide whether $|z'|>1-r $ or $|z'|<1-r$.  If $|z'|>1-r $, then compute $f(z')$ at precision $\varepsilon/2$. By Warshawsky's theorem, this is an $\varepsilon$ approximation of $\bar{f}(z)$.  If $|z'|<1-r$, then $z\in D$, and therefore we can just compute $f(z)$.  

For the converse, assume we are given $\bar{f}$. Since $\bar{D}$ is computably compact, we can compute  the modulus of continuity of $\bar{f}$:
 $$h(\delta):=\sup_{z,z'\in \bar{D}}|f(z)-f(z')|.$$ 
 
 Computability of the rate decay of  $\eta(\delta)$ now follows from Corollary \ref{ContinuityToCaratheodory}.

 

 
\end{proof}



 
The following result shows that even if  $\eta$ and $m$ account for the same geometric property, they are computationally different.  In particular, the corresponding rates of decay  are computationally incommensurable. 

\begin{theorem}[Incommensurability  of the  moduli]
There is a computable locally connected domain $U$ such that $\eta(\delta)$ has a computable rate decay whereas  $m(\delta)$ doesn't. 
\end{theorem}

\begin{proof}Let $B\subset \NN$ be a computable enumerable, non computable set.  
Let $I$ be the square  centred at the origin, with length  side equal to 2. Let $x_{i}=1-1/i$. The boundary $\partial U$ is constructed by modifying $I$ as follows.  If $i\notin B$, then add a straight line to $I$  from $(x_{i},1)$ to $(x_{i},x_{i})$. Call these  $i$-lines.  If $i\in B$ and it is enumerated in stage $s$, then remove the segment from $(x_{i}-s_{i},1)$ to $(x_{i}+s_{i},1)$ where $s_{i}=\min\{2^{-s}, 1/(3i^{2})\}$. To close the domain, join by straight lines $(x_{i}-s_{i},1)$ to $(x_{i}-s_{i},x_{i})$  to $(x_{i}+s_{i},x_{i})$ to $(x_{i}+s_{i},1)$. Call these $i$-fiords.  This completes the construction of $U$. We now show how to compute a $2^{-s}$ Housdorff approximation of the boundary. Start by running the machine enumerating $B$ for $s+1$ steps. For all those $i$'s that have been enumerated so far, draw the corresponding $i$-fiords.  For all the other $i$'s, draw a $i$-line. This is clearly a $2^{-s}$ approximation of $U$ since for any $i$ enumerated after the $s+1$ steps, the Hausdorff distance between the $i$-line and the $i$-fiord is less than $2^{-s}$. The Caratheodoty modulus is clearly computable. For example we can take $\eta(\delta)=2\sqrt \delta$ ($\delta<1)$. Assume that the modulus of connectivity $m(\delta)$ is also computable. That is, if $|x-y|<m(\delta)$, then diam$\gamma_{x\to y} < \delta$. For $i,n\in \NN$ let $x(i,n)= x_{i}-m(1/n)/2$ and $y(i,n)=x_{i}+m(1/n)/2$. Then diam$\gamma_{x(i,n)\to y(i,n)}<1/n$ which implies that no $i<n$ can be in $B$. A contradiction. 
\end{proof}



\subsection{Computational complexity on the boundary}We now discuss the computational complexity of computing $\bar{\varphi}$ and $\bar{f}$.  For $\bar{\varphi}$ we construct, for any  given computable function $\phi(n)$, a Jordan domain for which time complexity is greater than $\phi(n)$.  For $\bar{f}$ we show that its time complexity is bounded by below by the time complexity of the Caratheodory modulus, and therefore it can be arbitrarily high as well. 


\begin{theorem}
The computational complexity of both $\bar{\varphi}$ and $\bar{f}$ can be arbitrarily high.
\end{theorem}

\begin{proof}

The idea is to produce a domain $U$ with Jordan boundary $\partial U$ such that there is a sequence of points $w_{n}$ in $\partial U$, satisfying for instance $w_{n}\to w$ and $|w_{n}-w_{n+1}|=2^{-{\phi(n)}}$, whereas the corresponding points $z_{n}=\bar{\varphi}(w_{n})$ in $\partial D$ satisfy $|z_{n}-z_{n+1}|\geq 2^{-n}$. By observing that  at least $\phi(n)+1$ bits are needed to separate $w_{n}$ from $w_{n+1}$ (and therefore $\phi(n)+1$ computer steps), one sees that $\phi$ is a lower bound for  the time complexity of  $\bar{\varphi}$.  Indeed, only $n+1$ bits are needed to separate $z_{n}$ from $z_{n+1}$.  The second assertion follows from Corollary \ref{ContinuityToCaratheodory}.
\end{proof}

















